Duplicate-sensitivity Guided Transformation Synthesis for DBMS Correctness Bug Detection

Database Management System (DBMS) plays a core role in modern software from mobile apps to online banking. It is critical that DBMS should provide correct data to all applications. When the DBMS returns incorrect data, a correctness bug is triggered. Current production-level DBMSs still suffer from insufficient testing due to the limited hand-written test cases. Recently several works proposed to automatically generate many test cases with query transformation, a process of generating an equivalent query pair and testing a DBMS by checking whether the system returns the same result set for both queries. However, all of them still heavily rely on manual work to provide a transformation which largely confines their exploration of the valid input query space. This paper introduces duplicate-sensitivity guided transformation synthesis which automatically finds new transformations by first synthesizing many candidates then filtering the nonequivalent ones. Our automated synthesis is achieved by mutating a query while keeping its duplicate sensitivity, which is a necessary condition for query equivalence. After candidate synthesis, we keep the mutant query which is equivalent to the given one by using a query equivalent checker. Furthermore, we have implemented our idea in a tool Eqsql and used it to test the production-level DBMSs. In two months, we detected in total 30 newly confirmed and unique bugs in MySQL, TiDB and CynosDB.

==> background.tex <==
% \section{Background}
% In this section, We introduce automated DBMS testing and the related concepts.

% \textbf{Automated DBMS Testing (ADBT).} We limit the scope of this paper in ADBT, to differentiate it from many other works on database system testing. Specifically, ADBT refers to an automatic process, where a system could automatically generate test cases, run the tests and verify the test results. To automatically test the DBMS, the system should generate a test case of three elements: a database, a query and a testing oracle. We call the first two elements as inputs to the test case. 

% \textbf{Testing Oracle for ADBT.} A testing oracle is an expected return result from executing the query on the database. However, it is not easy to obtain an oracle in our scenario. SQL is highly expressive and every vendor has its own implementation f the language. This makes it hard to verify execution result for a query by comparing execution results from different systems. Similarly, metamorphic testing \cite{02metamorphic} must use existing test cases to construct new ones, which heavily relies on the usability of 
